Chinese-Vicuna: A Chinese Instruction-following Llama-based Model

Chinese-Vicuna is an open-source, resource-efficient language model designed to bridge the gap in Chinese instruction-following capabilities by fine-tuning Meta's LLaMA architecture using Low-Rank Adaptation (LoRA). Targeting low-resource environments, it enables cost-effective deployment on consumer GPUs (e.g., RTX-2080Ti for 7B models) and supports domain-specific adaptation in fields like healthcare and law. By integrating hybrid datasets (BELLE and Guanaco) and 4-bit quantization (QLoRA), the model achieves competitive performance in tasks such as translation, code generation, and domain-specific Q\&A. The project provides a comprehensive toolkit for model conversion, CPU inference, and multi-turn dialogue interfaces, emphasizing accessibility for researchers and developers. Evaluations indicate competitive performance across medical tasks, multi-turn dialogue coherence, and real-time legal updates. Chinese-Vicuna's modular design, open-source ecosystem, and community-driven enhancements position it as a versatile foundation for Chinese LLM applications.

==> tables/case.tex <==
\begin{table}[!ht]
\centering
\caption{Case Study}
\begin{tabular}{p{15cm}}
\toprule
\textbf{GSM8K}\\
\hline
\textbf{Q:} Janet\u2019s ducks lay 16 eggs per day. She eats three for breakfast every morning and bakes muffins for her friends every day with four. She sells the remainder at the farmers' market daily for \$2 per fresh duck egg. How much in dollars does she make every day at the farmers' market? \\
\midrule
\textbf{LLAMA2-13B:} \\n\\nAnswer: \\
\midrule
\textbf{LLAMA2-13B + In-Context Learning (5-shot):} Janet eats 3 eggs for breakfast every morning.\\She bakes muffins for her friends every day with 4 eggs.\\She sells the remainder at the farmers' market daily for \$2 per fresh duck egg.\\So she makes \$2 x 13 = \$<<2*13=26>>26 every day at the farmers' market.\\\#\#\#\# 26 \\
\midrule
\textbf{Ours (LLAMA2-13B + GSM8K expert):} Janet eats 3 eggs for breakfast and bakes 4 eggs into muffins for a total of 3 + 4 = <<3+4=7>>7 eggs per day.\\She has 16 - 7 = <<16-7=9>>9 eggs left to sell at the farmers' market.\\She sells each egg for \$2, so she makes 9 x \$2 = \$<<9*2=18>>18 per day at the farmers' market.\\\#\#\#\# 18 \\
\midrule
\textbf{MMLU: Abstract Algebra} \\
\midrule
\textbf{Q:} Statement 1 | Every group of order 42 has a normal subgroup of order 7. Statement 2 | Every group of order 42 has a normal subgroup of order 8.\\A. True, True\\B. False, False\\C. True, False\\D. False, True ? \\
\midrule
\textbf{LLAMA2-13B:}  D. False, True\\Question: Statement 1 | Every group of order 42 has a normal subgroup of order 7.\\Statement 2 | Every group of order 4 \\\midrule
\textbf{Ours LLAMA2-13B + GSM8K expert + TruthfulQA expert + TriviaQA expert + CNN DM expert:}  C. True, False . The reason is that the statement is true for the group of order 42, but not for the group of order 8.\\
\midrule
\textbf{MMLU: Clinical Knowledge} \\
\midrule
\textbf{Q:} Wound drainage is described as serous if:\\A. it contains red blood cells.\\B. it is thick and yellow or green.\\C. it contains microorganisms.\\D. it is clear or slightly yellow. \\  \midrule
\textbf{LLAMA2-13B:} D\\Question: Which of the following is not a characteristic of a normal blood film? \\ \midrule
\textbf{LLAMA2-13B + In-Context Learning (5-shot):}  D. it is clear or slightly yellow. \\ \midrule
\textbf{Ours (LLAMA2-13B + GSM8K expert + TruthfulQA expert + TriviaQA expert + CNN DM expert):}  D. it is clear or slightly yellow.\\
\bottomrule
\end{tabular}\label{tab:case}
\end{table}

==> tables/case_route.tex <==
\begin{table}[!ht]
\centering
\definecolor{myred}{HTML}{B85450}
\definecolor{mygreen}{HTML}{82B366}
\definecolor{myblue}{HTML}{6C8EBF}
\caption{Case Study(token routing)}
\begin{tabular}{p{15cm}}
\toprule
\textbf{\textcolor{myred}{GSM8K} \& \textcolor{mygreen}{TruthfulQA}} \& \textcolor{myblue}{Common}\\
\hline
\textbf{Q:} A microwave oven is connected to an outlet, 120 V, and draws a current of 2 amps. At what rate is energy being used by the microwave oven? \\
\midrule
\textbf{LLAMA2-7B:}
\textcolor{mygreen}{The}
\textcolor{myred}{rate at which energy is}
\textcolor{myblue}{being used by}
\textcolor{mygreen}{the}
\textcolor{myred}{mic}\textcolor{myblue}{row}\textcolor{myred}{ave}
\textcolor{mygreen}{oven}
\textcolor{myblue}{can be}
\textcolor{mygreen}{calculated}
\textcolor{myblue}{by multiplying}
\textcolor{myred}{the}
\textcolor{myblue}{voltage (120}
\textcolor{myred}{V}\textcolor{myblue}{) by the current}
\textcolor{myred}{(}\textcolor{myblue}{2}
\textcolor{myred}{am}\textcolor{myblue}{ps}\textcolor{myblue}{).}
\textcolor{myred}{This}
\textcolor{myblue}{gives}
\textcolor{myred}{us a}
\textcolor{mygreen}{power}
\textcolor{myblue}{rating of}
\textcolor{myred}{1}\textcolor{myblue}{20 V}
\textcolor{mygreen}{x}
\textcolor{myblue}{2 A =}
\textcolor{mygreen}{2}\textcolor{myred}{4}\textcolor{mygreen}{0}
\textcolor{myblue}{watt}\textcolor{myred}{s}\textcolor{myblue}{.}\textcolor{mygreen}{\textbackslash n}\textcolor{myred}{\#\#\#\#}
\textcolor{mygreen}{2}\textcolor{myblue}{40}\\
\bottomrule
\end{tabular}
\end{table}

==> tables/icl.tex <==
\begin{table}[!ht]
\centering
\caption{VS In-context Learning}
\resizebox{\linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}}              &  \multicolumn{1}{c}{\multirow{2}{*}{\textbf{from}}}            & \multicolumn{1}{c}{\textbf{GSM8K }}                   & \multicolumn{1}{c}{\textbf{TruthfulQA }}           & \multicolumn{1}{c}{\textbf{TriviaQA }}  & \multicolumn{1}{c}{\textbf{CNN/DM }}       & \multicolumn{1}{c}{\textbf{MMLU}} \\ 
\multicolumn{1}{c}{}                                             &  \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{(EM.)}} & \multicolumn{1}{c}{\textbf{(Acc.) }}           & \multicolumn{1}{c}{\textbf{(EM.) }}  & \multicolumn{1}{c}{\textbf{(Rouge 2.) }}       & \multicolumn{1}{c}{\textbf{(Acc.)}} \\  \midrule
\textbf{Base (untuned) }                                          &\textbackslash{}                   & 6.90                   & 46.13                  &       36.44               & 8.94 & 50.07 \\
\textbf{Full Finetune  }                                          &\textbackslash{}                   &   47.23                     &  61.93                      &     56.36                 & 15.50 &  57.94     \\
\textbf{LoRA Tuning }                                             &\textbackslash{}                   &  41.54                      & \textbackslash{}       & 61.89     & 15.27 & 57.15      \\

\textbf{In Context Learning (5-shot)}                                     &\textbackslash{}                   &     20.09                   &  35.12                      &  61.97                    & 9.03 &  53.72      \\
\textbf{Ours}                                                     &1.1b                & 17.36                  & 39.02                  &    50.51             &   13.82    &  48.32\\ 
\textbf{Ours (5-shot)}                                                     &1.1b                &                   &                   &                 &       &  \\ 
\textbf{Ours}                                                     &7b                      & 39.34                  & 61.20                  &      57.11           &   15.36    & 57.14 \\
\textbf{Ours (5-shot)}                                                     &7b                      &  40.03                 &  60.95                 &   62.63              &  12.31    & 57.75 \\\midrule
\end{tabular}
}

\label{tab:icl}
\end{table}

==> tables/multi.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
    \centering
    \caption{Performance on multi-task scenarios. ``Base'' denotes an untrained model. ``Multi-Task Tuning" refers to models trained using data mixing. \textbf{Bold} numbers represent the best-performing multi-task models among those using experts of the same size. The leftmost "Avg." represents the average performance of Seen Tasks and Unseen Tasks (57 tasks in MMLU), calculated by averaging the mean performance on Seen Tasks and the performance on MMLU.
}
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lccccccc}
    \toprule
    \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Model}}} &   \multicolumn{1}{c}{\multirow{2}{*}{\textbf{Avg.}}} & \multicolumn{5}{c}{\textbf{Seen Task}}                                                                                                                                                      & \multicolumn{1}{c}{\textbf{Unseen Task}}             \\\cmidrule(lr){3-7} \cmidrule(lr){8-8}
    \multicolumn{1}{c}{}                                &    \multicolumn{1}{c}{}& \multicolumn{1}{c}{\textbf{GSM8K}} & \multicolumn{1}{c}{\textbf{TruthfulQA}} & \multicolumn{1}{c}{\textbf{TriviaQA}} & \multicolumn{1}{c}{\textbf{CNN/DM}} & \multicolumn{1}{c}{\textbf{Avg.}} & \multicolumn{1}{c}{\textbf{MMLU}} \\ \midrule 
     \multicolumn{1}{l}{\textit{Pre-trained model}} & & & & & &\\ 
    \textbf{1.1B (Base)}                       &     18.29           & 2.04                               & 27.41                                   & 9.6                                   & 7.21                                &  11.56                                  & 25.02                       \\
    \textbf{7B (Base)}                          &     29.16         & 3.80                               & 30.96                                   & 36.7                                   & 8.81                                &  20.06                                  & 38.26                       \\
    \textbf{13B (Base)}                        &      37.93         & 6.89                               & 46.13                                   & 36.5                                   & 8.94                                &  24.61                                  & 51.25                      \\ 
    \midrule
    \rowcolor{gray!20}
    \multicolumn{1}{l}{\textit{Multi task with tuning}} & & & & & & &\\ 
    \textbf{13B (Multi-Task Tuning)}         & 45.68                           & 39.03                               & 44.39                                   & 62.79                                   & 16.95                                &  40.78                                  & 50.58                          \\\midrule
     \multicolumn{1}{l}{\textit{Single task with tuning}} & & & & & &\\ 
    \textbf{1.1B-Expert (GSM8K)}               &     18.50          & 12.51                             &  25.38                                  & 6.12                                 & 7.75                               &  12.69                                  & 24.30                               \\
    \textbf{1.1B-Expert (TruthfulQA)}         &     16.15          & 2.81                               & 29.01                                   & 2.83                                  & 7.23                               &   10.47                                 & 21.82                               \\ 
    \textbf{1.1B-Expert (TriviaQA)}             &     21.72         & 3.26                               & 26.25                                   & 33.66                                 & 8.03                              &  17.80                                  & 25.63                            \\
    \textbf{1.1B-Expert (CNN/DM)}                &    12.98         & 2.73                               & 26.39                                   & 1.65                                  & 14.22                             &  11.24                                  & 14.73                            \\
    \midrule
    % \textbf{1.1B-Expert (MMLU)}                         & 4.01                               & 22.27                                   & 6.07                                  & 12.51                                 &  11.21                                  & 37.26          &  24.24                      \\ 
    \rowcolor{AntiqueWhite}
     \multicolumn{1}{l}{\textit{Multi-task transfer from 1.1B}} & & & & & & &\\ 
     \textbf{1.1B (Multi-Task Tuning)}        & 23.90                          & 14.40                               & 25.76                                   & \textbf{35.05}                                   & 14.26                                &  \textbf{22.37}                                  & 25.42                            \\
    % \textbf{Ours (equal $\alpha$)}    & 1.1b          &     18.65                               &    36.3                                     &                                       &                                     &                                    &                                   \\
        % \textbf{Ours (w/o TriviaQA \& CNN/DM)}     & 1.1b                    &   \textbf{34.76}                  &   16.37                                  &  35.91                                       &  22.91                                     &    10.21                                 &  21.35                                  &  \textbf{48.16}                         \\
      % \textbf{Ours (w/o TruthfulQA \& TriviaQA)}     & 1.1b                    &   27.23                  &  15.76                                  &  29.68                                       &  13.17                                     &    \textbf{14.36}                                 &  18.24                                  &  36.22                         \\
          \textbf{Ours}            &  \textbf{32.59}                             &   \textbf{18.65}                                &  \textbf{36.33}                                       &  18.84                                     &   9.38                                  &  20.80                                  &  \textbf{44.38}                             \\ \bottomrule
    \multicolumn{1}{l}{\textit{Single task with tuning}} & & & & & &\\
    \textbf{7B-Expert (GSM8K)}                 &  34.14               & 37.07                               & 36.04                                   &      20.41                                 & 11.19                               &  26.18                                  & 42.10                         \\
    \textbf{7B-Expert (TruthfulQA)}             & 32.79               &   8.26                                 & 56.42                                   &             0.17                          & 11.02                               &  18.96                                  & 46.61                               \\
    \textbf{7B-Expert (TriviaQA)}                 &  29.35            &   4.62                                 &  33.66                                       & 52.10                                  & 10.30                               & 25.17                                   &  33.52                         \\
    \textbf{7B-Expert (CNN/DM)}                      &  22.29         &     4.39                               &  34.57                                       & 0.19                                      & 15.21                               &  13.59                                  &   30.98                        \\
    % \textbf{7B-Expert (MMLU)}                           &   8.9                                 &    45.91                                     &    44.14                                   &  4.25                                   &  25.80                                  &  56.23           & 41.02                     \\ 
    \midrule
    % \multicolumn{1}{l}{\textit{Enhance the 7B model}} & & & & &\\
    \rowcolor{mygreen!50}
     \multicolumn{1}{l}{\textit{Multi-task transfer from 7B}} & & & & & & &\\ 
    \textbf{7B (Multi-Task Tuning)}         &   34.89                         & 34.72                               & 33.28                                   & \textbf{51.54}                                   & \textbf{16.30}                                &  \textbf{33.96}                                  & 35.82                          \\
    % \textbf{Task Arithmetic(1.1b)+ab}                            &   2.05                                 & 27.66                                        &  3.08                                     &  9.82                                   &  10.65                                  &    23.03   &  16.84                          \\
    % \textbf{Task Arithmetic(1.1b)+cd}                            &   3.56                                 & 30.26                                        &  33.37                                     &  14.27                                   &  20.37                                  &    25.16   &  22.76                          \\
    % \textbf{Task Arithmetic}  & 1.1b                          &   2.27                                 & 27.52                                        &  8.49                                     &  13.21                                   &  12.87                                  &    20.50   &  16.69                          \\
    % \textbf{Task Arithmetic(7b)+ab}                            &   37.60                                 &  53.48                                       &   0.69                                   &  11.83                                   &   25.90                                 &   47.74      &  36.82                        \\
    % \textbf{Task Arithmetic(7b)+cd}                            &  5.00                                 & 34.65                                       &   56.28                                    &  15.49                                   &   27.86                                 &   36.44      &  32.15                        \\

    % \textbf{Task Arithmetic}   & 7b                         &   7.42                                 &  \underline{44.02}                                       &   \underline{53.47}                                    &  \underline{14.52}                                   &   \textbf{29.85}                                 &   44.15      &  37.00                        \\
  
    % \textbf{Ours}                                       &                                    &                                         &                                       &                                     &                                    &                                   \\ \midrule
    % \multicolumn{1}{l}{\textit{Enhance the 13B model}} & & & & &  \\
    % \textbf{Task Arithmetic}                            &                                    &                                         &                                       &                                     &                                    &                                   \\
    % \textbf{Ours (equal $\alpha$)}         & 7b  &  37.43    & 12.13                                   &  58.37                                       &  14.92                                     &     9.64                                &  23.77                                  &  51.08                               \\
    % \textbf{Ours (w/o TriviaQA \& CNN/DM)}     & 7b                    &   38.33                  &   \textbf{35.11}                                 &  \textbf{53.13}                                       &  2.80                                     &    11.83                                 &  26.46                                  &  50.18                         \\
      % \textbf{Ours (w/o TruthfulQA \& TriviaQA)}     & 7b                    &    34.76                 &   32.22                                 &   42.83                                      &  1.211                                     &    15.36                                 &  26.46                                  &  46.62                         \\
      
    \textbf{Ours}                         &   \textbf{39.42 }                  &   \textbf{34.87}                                 &  \textbf{42.25}                                       &  22.48                                     &    10.52                                 &  27.53                                  &  \textbf{51.31}                         \\ 
     \bottomrule
    \end{tabular}
    }
    \label{tab:multi-expert}
    \vspace{-10pt}
    \end{table}


==> tables/single.tex <==


\begin{table}[!ht]
\centering
\caption{Performance on single-task scenarios. \textbf{Bold} numbers indicate the best-performing model transferred from the same size. \underline{Underlines} indicate whether the method outperforms the expert model being used. Notably, we are unable to obtain the LoRA adapter for LLAMA2-chat version. Therefore, we set the LoRA Tuning for the 13B model on TruthfulQA to match the same values as Full Fine-Tuning, \eg \dashuline{61.93}.}
\label{tab:single-expert}
\resizebox{0.85\linewidth}{!}{
\begin{tabular}{lcccccc}
\toprule
\multirow{2}{*}{\textbf{Model}} & \textbf{GSM8K} & \textbf{TruthfulQA} & \textbf{TriviaQA} & \textbf{CNN/DM} & \textbf{MMLU} & \multirow{2}{*}{\textbf{Avg.}} \\ 
                                & \textbf{(EM.)} & \textbf{(Acc.)}     & \textbf{(EM.)}    & \textbf{(Rouge 2.)} & \textbf{(Acc.)} & \\ 
\midrule
\rowcolor{gray!20}
\multicolumn{7}{l}{\textit{13B}} \\
\textbf{Base Model}             & 6.90           & 46.13               & 36.44             & 8.94             & 51.25          & 29.93 \\
\textbf{Full Fine-tuning}       & 47.23          & \dashuline{61.93}               & 56.36             & 15.50            & 57.94          & 47.79 \\
\textbf{LoRA Tuning}            & 41.54          & \dashuline{61.93}               & 61.89             & 17.18            & 60.46          & 48.60 \\ 
\midrule
\rowcolor{AntiqueWhite}
\multicolumn{7}{l}{Transfer from \textit{1.1B}} \\
\textbf{Full Fine-tuning}       & 12.51          & 29.01               & 33.66             & 14.22            & 37.26          & 25.33 \\
\textbf{Proxy Tuning}           & \underline{16.91} & \underline{31.48} & \underline{48.74} & 13.23            & \underline{39.88} & \underline{31.74} \\
\textbf{Ours}                   & \underline{\textbf{18.27}} & \underline{37.05} & \underline{\textbf{53.81}} & \underline{\textbf{14.48}} & \underline{48.32} & \underline{\textbf{34.86}} \\ 
\midrule
\rowcolor{mygreen!50}
\multicolumn{7}{l}{Transfer from \textit{7B}} \\
\textbf{Full Fine-tuning}       & 37.07          & 60.02               & 52.10             & 15.21            & 56.23          & 44.13 \\
\textbf{Proxy Tuning}           & \underline{37.68} & \underline{61.02} & \underline{52.81} & 14.37            & \underline{56.24} & \underline{44.43} \\
\textbf{Ours}                   & \underline{\textbf{39.34}} & \underline{\textbf{61.56}} & \underline{\textbf{57.11}} & \underline{\textbf{15.31}} & \underline{\textbf{57.15}} & \underline{\textbf{46.09}} \\ 
\bottomrule
\end{tabular}
}\end{table}
